Stability and Resilience of Distributed Information Spreading in Aggregate Computing

Spreading information through a network of devices is a core activity for most distributed systems. As such, self-stabilizing algorithms implementing information spreading are one of the key building blocks enabling aggregate computing to provide resilient coordination in open complex distributed systems. This paper improves a general spreading block in the aggregate computing literature by making it resilient to network perturbations, establishes its global uniform asymptotic stability and proves that it is ultimately bounded under persistent disturbances. The ultimate bounds depend only on the magnitude of the largest perturbation and the network diameter, and three design parameters trade off competing aspects of performance. For example, as in many dynamical systems, values leading to greater resilience to network perturbations slow convergence and vice versa.

==> arxiv preprints/simulations.tex <==


In this section, we empirically confirm the results presented in the prior sections through simulations.
We first investigate the effect of parameters in the general spreading block configured as GABF, then compare with the performance of ABF in the presence of persistent perturbations. 
Finally, we illustrate the applicability of the general spreading block to more complex cases with an example of a non-Euclidean distance metric.
%
Except where otherwise noted, all simulations use 500 nodes, randomly distributed in a 4 km $\times$ 1 km area, and communicating via broadcast within a 0.25 km radius. 
One node is designated as a source and initial distance estimates of all nodes follow a uniform distribution between 0 and $\sqrt{17}$ km (i.e., the longest possible distance for the simulated space).

\subsection{Effect of parameters}

We begin with an empirical investigation of the design choices and parameter effects discussed in Section~\ref{sdesign}, using GABF, as defined in Section \ref{sgalg}, as an example to demonstrate the impact of these parameters  on  convergence speed. 

Progress toward convergence may be measured using the greatest overestimate $\Delta^+(t)$ and least underestimate $\Delta^-(t)$:
\begin{eqnarray}
\Delta^+(t) & = & \max\left [0,\max_{i} \left\{\Delta_i(t) \right\}\right ]\label{D+}\\
\Delta^-(t) & = & \max\left [0,-\min_{i} \left\{ \Delta_i(t) \right\} \right ].\label{D-}
\end{eqnarray}
where $\Delta_i(t)=\hat{d}_i(t)-d_i$ the distance estimation error of node $i$. Then $\Delta^+(t) = \Delta^-(t) = 0$ indicates that all distance estimates converge to their true distances at time $t$.

% run 100 times
%%%%%%%%%%%%%%%%%%%%%%
% \delta

\begin{figure}
	\centering
	\subfigure[$\Delta^+(t)$]{
		\includegraphics[width = 1\columnwidth]{envelopeDeltaP.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$]{  
		\includegraphics[width = 1\columnwidth]{envelopeDeltaM.pdf}}
	\caption{Convergence time for (a) the greatest overestimate $\Delta^+(t)$ and (b) the least underestimate $\Delta^-(t)$ without perturbations, with $M = 5$, $D = 0$ and $\delta$ is varying from $0.2M$ to $M$ in steps of $0.2M$. The solid line represents the average value of 100 trials, the dotted and dashed lines represent upper and lower envelopes, respectively. 
	In (b) solid and dotted lines of $\delta = 0.8M$ and $\delta = M$ overlap, and dashed lines of $\delta = 0.4M$, $\delta = 0.6M$, $\delta = 0.8M$ and $\delta = M$ overlap.}
	\label{fig:delta}
\end{figure} 

We start with $\delta$, which controls how quickly $M$ is reached.
Figure~\ref{fig:delta} shows the results of 100 runs using $M = 5$, $D = 0$, and $\delta$ varying from $0.2M$ to $M$ in steps of $0.2M$.
The average $\cD(\cG)$ is 18.8.
With a fixed $M$, both $\Delta^+(t)$ and $\Delta^-(t)$ converge slower with a smaller $\delta$, since a smaller $\delta$ means estimates exceed $M$ later.
The corresponding average convergence times are 61.2, 54.1, 38.1, 32.6 and 24.1.
%(in Figure \ref{fig:delta} (b) solid and dotted lines of $\delta = 0.8M$ and $\delta = M$ overlap, and dashed lines of $\delta = 0.4M$, $\delta = 0.6M$, $\delta = 0.8M$ and $\delta = M$ overlap). 
 
%%%%%%%%%%%%%%%%%%%%%%
% D

\begin{figure}
	\centering
	\subfigure[$\Delta^+(t)$]{
		\includegraphics[width = 1\columnwidth]{envelopeDP.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$]{  
		\includegraphics[width = 1\columnwidth]{envelopeDM.pdf}}
	\caption{Convergence time for (a) the greatest overestimate $\Delta^+(t)$ and (b) the least underestimate $\Delta^-(t)$ without perturbations, with $\delta = M = 5$ and $D = 0, 0.01K, 0.1K, K$ and $4K$, using $K = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$. The solid line represents the average value of 100 trials, the dotted and dashed lines represent upper and lower envelopes, respectively. 
	In (b) dashed lines of $D = 0, 0.01K$ and $0.1K$ overlap.}
	\label{fig:D}
\end{figure} 

The dead zone value $D$, on the other hand, has opposing effects on $\Delta^+(t)$ and $\Delta^-(t)$.
Figure~\ref{fig:D} shows the results of 100 runs using $\delta = M = 5$ and $D = 0, 0.01K, 0.1K, K$ and $4K$, using $K = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$.
In these simulations, the average value of $\epsilon$ is $2.5 \times 10^{-3}$ km and the average values of $\cD(\cG)$ and $\cD(\cG^-)$ are 17.9 and 26.8, respectively.
%
For $\Delta^+(t)$, a large $D$ (e.g., $D = 4K$) or a small $D$ (e.g., $D = 0$) accelerates convergence. 
In the former case GABF acts more like ABF in which case $\cD(\cG)$ will converge within $\cD(\cG) - 1$ rounds \cite{TAC}. In the latter case the second bullet of (\ref{raising}) will be frequently invoked such that underestimates will be eliminated more quickly with a large $M$, and thus $T$ defined in (\ref{tstar}) becomes smaller. 
Both of these phenomena are seen in these simulations, with the average convergence time of $\Delta^+(t)$ being 23.2, 67.9, 99.3, 34.0 and 6.5. 
%
As for $\Delta^-(t)$, A large $D$ always has a negative impact on the convergence speed of $\Delta^-(t)$ since the behavior of GABF is more like ABF in this situation, where the \emph{rising value problem} \cite{TAC,mo2018robust} will cause the underestimates rise very slowly.
Here, the average convergence time is 2, 49.3, 310.0, 535.9 and 631.7.
Note that these underestimates are more vulnerable to the change of $D$: while the time to convergence of $\Delta^+(t)$ is roughly 60 rounds faster by increasing $D$ from $0.1K$ to $K$, that of $\Delta^-(t)$ may be hundreds of rounds slower under such a change. 
%
Overall convergence time is thus regulated by $\Delta^+(t)$ for small $D$ and by $\Delta^-(t)$ for large $D$, with the joint average convergence time of 23.2, 67.9, 310.0, 535.9 and 631.7.

%%%%%%%%%%%%%%%%%%%%%%
% M
\begin{figure}
	\centering
	\subfigure[$\Delta^+(t)$]{
		\includegraphics[width = 1\columnwidth]{envelopePM.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$]{  
		\includegraphics[width = 1\columnwidth]{envelopeMM.pdf}}
	\caption{Convergence time for (a) the greatest overestimate $\Delta^+(t)$ and (b) the least underestimate $\Delta^-(t)$ without perturbations, with $D = 0$, $\delta = M$, and $M$ varying from 4.108 to 4.124. The solid line represents the average value of 100 trials, the dotted and dashed lines represent upper and lower envelopes, respectively. 
	In (b) dashed lines of all different M overlap, and dotted lines of $M = 4.108$ and $4.112$ overlap.}
	\label{fig:M}
\end{figure} 

Finally, the impact of $M$ may be separated out from the other two parameters by setting $D=0$ and $\delta=M$.
In this condition, small changes in $M$ can result in large changes in convergence rate.
%
Figure~\ref{fig:M} illustrates this for 100 runs of GABF, with $D=0$, $\delta=M$, and $M$ increasing from 4.108 to 4.124 in steps of 0.004.
In these simulations, the average $\cD(\cG)$ is 18.5.
Here, convergence unconditionally improves with higher $M$: the average convergence times of $\Delta^+(t)$ are 92.9, 72.6, 55.1, 32.0 and 23.7 rounds, while those of $\Delta^-(t)$ are 87.3, 63.0, 43.5, 14.4 and 2 rounds.
%
Even though $T_i$ defined in (\ref{ti}) satisfies $T_i = 3$ for all different $M$, as we have set $\delta = M$, overestimates disappear more quickly with larger $M$ because a larger $\delta$ helps the time $T$ defined in (\ref{tstar}), after which all states are overestimates becoming smaller by (\ref{eq:ude}) in Lemma \ref{luin}. 
Underestimates converge more quickly once $M$ is greater than both the largest true distance and initial distance estimate. In this case, all nodes acquire overestimates in the first round by invoking the second bullet of (\ref{raising}),
and thus the underestimates converge in only 2 rounds.

\subsection{Robustness against persistent perturbations}

\begin{figure}
	\centering
	\subfigure[$\Delta^+(t)$ and $(\cD(\cG) - 1)\epsilon$]{
		\includegraphics[width = 0.94\columnwidth]{perP.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$ and $(\cD(\cG^-) - 1)\epsilon$]{  
		\includegraphics[width = 0.94\columnwidth]{perM.pdf}}
	\caption{Robustness against perturbation for GABF with various values of $D$, compared over 100 trials with ultimate bounds and with ABF: (a) mean values of $\Delta^+(t)$ and mean value of ultimate bound $(\cD(\cG) - 1)\epsilon$, and (b) mean values of $\Delta^-(t)$ and mean value of ultimate bound $(\cD(\cG^{-}) - 1)\epsilon$. Edge lengths are perturbed by measurement errors uniformly distributed between 0 and $e_{\min}$. Parameters for GABF are set as $\delta = M = \sqrt{17}$, $D = 0, 0.02K, 0.05K, 0.2K, 0.4K, K$ and $2K$, where $K = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$. In (a), lines of $D = 0, 0.02K$ and $0.05K$ overlap.}
	\label{fig:perturbation}
\end{figure} 

As discussed in Section~\ref{sdesign}, robustness against perturbation should be controlled primarily by parameter $D$.
In particular, $(\cD(\cG)-1)\epsilon$ and $(\cD(\cG^-)-1)\epsilon$ are the ultimate bounds of $\Delta^+(t)$ and $\Delta^-(t)$ under perturbations, respectively \cite{TAC} (i.e., $L_1W(L_2,\cD(\cG)-1)$ and $L_1W(L_2,\cD(\cG^-)-1)$ in Theorem \ref{tpre}, respectively), and thus $(\cD(\cG) + \cD(\cG^-) - 2)\epsilon$ is the minimum value of $D$ to guarantee the robustness of GABF under perturbations. 

Figure \ref{fig:perturbation} illustrates this for 100 runs of GABF, comparing this ultimate boundedness with ABF and with GABF using $\delta = M = \sqrt{17}$ and $D = 0, 0.02K, 0.05K, 0.2K, 0.4K, K$ or $2K$, where $K = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$, $\epsilon = 0.05e_{\min}$.
Perturbation is injected as asymmetric noise in the estimated $e_{ij}$, such that measurement errors $\epsilon_{ij}(t)$ defined in (\ref{vare}) follow a uniform distribution between 0 and $0.05e_{\min}$ in each round. 
In these simulations, the average value of $e_{\min}$ defined in (\ref{ep}) is $2.9 \times 10^{-3}$ km, $\cD(\cG) = 18.6$ and $\cD(\cG^-) = 20.0$ on average. 

The results show the tradeoffs in $\Delta^+(t)$ versus $\Delta^-(t)$ with GABF.
For $\Delta^-(t)$, ABF is constrained by the \emph{rising value problem} \cite{TAC,mo2018robust} such that $\Delta^-(t)$ needs a much longer time than $\Delta^+(t)$ to drop below than its ultimate bound.
With GABF, lower values of $D$ increase the speed of convergence, with $D=0$ achieving the fastest time.
%
For $\Delta^+(t)$, on the other hand, ABF converges extremely quickly, while GABF does not converge at all for low values of $D$.
In this case, GABF with $D = 0, 0.02K, 0.05K, 0.2K$ and $0.4K$ will not be ultimately bounded, while the average time for ABF and GBAF with $D = K$ and $2K$ to drop below the ultimate bounds follows 859.3, 196.5 and 300.1 rounds. Further, the average time for ABF and GABF with $D = K$ or $2K$ to reach the bottom is 5750 and 2406 rounds, respectively. 
Combining both, we find that GABF outperforms ABF under perturbations when the dead zone value $D$ is equal to or slightly larger than the minimum required value defined in (\ref{D}).
%
Thus, when the general spreading block is under perturbation, $D$ should be set as $(W(L_2,\cD(\cG^-) - 1) + W(L_2,\cD(\cG) - 1))L_1\epsilon$ defined in (\ref{D}) of Lemma \ref{tpre} in order to guarantee robustness and meanwhile attain a fast convergence speed. Observe though the floor is much below the theoretical ultimate bound, and even with $ D=.04K $, $ \Delta^+(t) $ though persistently rising from the floor rises only up to the unltimate bound.

%To gain more insights about the spreading block and the general spreading block, we now compare the performance of GABF and ABF in terms of the convergence speed. GABF uses two sets of parameters, one is with $\delta = M = \sqrt{17}$ km and $D = 0$, the other is with $\delta = M = \sqrt{17}$ km and $D = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$. The average $\cD(\cG)$ and $\cD(\cG)$ for those trials are 18.1 and 25.4, respectively, and $\epsilon$ is $2.0 \times 10^{-3}$ km on average. Figure \ref{fig:comparison} demonstrates the performances of GABF and ABF. The solid line depicts the average value for 100 trials, and the dotted and dashed lines in the same color depict the corresponding upper and lower envelopes, respectively. It can be seen that overestimates in ABF will decay within $\cD(\cG) - 1$ rounds, yet underestimates constrained by the \emph{rising value problem} need a much longer time to converge. The average convergence time for ABF is approximately 848.2 rounds. With $D = 0$, GABF is rid of the \emph{rising value problem} such that the underestimates will disappear within 2 rounds. Even though in this case the overestimates need slightly longer time to converge, the average convergence time of GABF is only 24.7 rounds, which is much shorter than that of ABF. Though compared with $D = 0$, the convergence time of GABF with $D = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$ becomes longer for the sake of robustness against perturbations, the average convergence time is 579.3 rounds, which is still roughly one-third shorter than ABF.
%
%\begin{figure}
%	\centering
%	\subfigure[$\Delta^+(t)$]{
%		\includegraphics[width = 0.94\columnwidth]{envelopeCP.eps}}
%	\vfill
%	\subfigure[$\Delta^-(t)$]{  
%		\includegraphics[width = 0.94\columnwidth]{envelopeCM.eps}}
%	\caption{Convergence time for (a) the greatest overestimate $\Delta^+(t)$ and (b) the least underestimate $\Delta^-(t)$ without perturbations. In this example, GABF is with two sets of parameters: $\delta = M = 5$, $D=0$, and $\delta = M = 5$, $D= (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$. The solid line represents the average value of 100 trials, the dotted and dashed lines in the same color represent the corresponding upper and lower envelopes, respectively.}
%	\label{fig:comparison}
%\end{figure} 

\subsection{Non-Euclidean Distance}

\begin{figure}
	\centering
	\subfigure[The spreading block of (\ref{spreading})]{
		\includegraphics[width = 0.8\columnwidth]{ABF.pdf}}
	\vfill
	\subfigure[The more general spreading block of (\ref{gengenG})-(\ref{raising})]{  
		\includegraphics[width = 0.8\columnwidth]{gabf.pdf}}
	\caption{In this example, 400 nodes are randomly located in a $4 \times 4$ $\mathrm{km}^2$ field. There is a source at the red asterisk located at (0.3, 0.3), and the middle of the field is a $2.5 \times 2.5$ $\mathrm{km}^2$ radiation zone. Color represents degree of contamination, with a logarithmic scale. While both spreading block and the general spreading block can achieve the shortest available path, the fast convergence of the general spreading block greatly reduces total contamination.}
	\label{fig:nonEuclidean}
\end{figure} 

Finally, we illustrate how the general spreading block can accommodate non-Euclidean distance metrics. 
Figure~\ref{fig:nonEuclidean} shows example of a  nonlinear $f(\cdot,\cdot)$ in (\ref{spreading}), for nodes to compute paths minimizing exposure to a hazard. In this scenario, 500 nodes are randomly distributed in a $4 \times 4$ $\mathrm{km}^2$ field, and communicate over a 0.6 km radius.  A source is located at (0.3, 0.3). In the middle of the area, there exists a $2.5 \times 2.5$ $\mathrm{km}^2$ \emph{radiation zone} centered at (1.95, 1.95). Define $\mathcal{M}$ as the set of nodes in the radiation zone, a node $i$ is radioactive if $i \in \mathcal{M}$ or $i$ has ever taken a radioactive node as its constraining node.  $f(\xh_k(t),e_{ik})$ in (\ref{spreading}) obeys $f(\xh_k(t),e_{ik}) = \xh_k(t) + e_{ik}, k \notin \mathcal{M}$, where $e_{ik}$ is the edge length between node $i$ and $k$. When $k \in \mathcal{M}$, $f(\xh_k(t),e_{ik}) = h(\xh_k(t) + 1000e_{ik})$, where $h(a) = a^{1.5}$ if $a > 1$ and $a$ otherwise. Further, $s_i$ defined in (\ref{spreading}) is 0 if $i$ is a source and $\infty$ otherwise. In each round a node $i$ will receive 100$\sim$120 units of radiation dose if it is radioactive and 0$\sim$1 unit otherwise. 
Figure~\ref{fig:nonEuclidean}(a) shows the result of using the spreading block defined in (\ref{spreading}), while Figure~\ref{fig:nonEuclidean}(b) shows the result from setting $D = 0, \delta = M > x_{\max}$ in the general spreading block. 
In both cases, nodes outside the radiation zone  never cross the zone due to the high cost, and nodes inside the zone  take the shortest path to exit the zone. However, the degree of contamination is greatly reduced when using the general spreading block with appropriately chosen parameters, due to the much faster time of convergence to a safe path.

%\begin{figure*}
%	\centering
%	\subfigure[$\Delta^+(t)$(GABF)]{
%		\includegraphics[width = 0.66\columnwidth]{dpGABF0.eps}}
%	\hfill
%	\subfigure[$\Delta^-(t)$(GABF)]{  
%		\includegraphics[width = 0.66\columnwidth]{dmGABF0.eps}}
%	\hfill
%	\subfigure[$\Delta^-(t)$(GABF)]{  
%		\includegraphics[width = 0.66\columnwidth]{dpgabfp.eps}}
%	\vfill
%	\subfigure[$\Delta^+(t)$(GABF)]{
%		\includegraphics[width = 0.66\columnwidth]{dmgabfp.eps}}
%	\hfill
%	\subfigure[$\Delta^+(t)$(ABF)]{
%		\includegraphics[width = 0.66\columnwidth]{dpABF.eps}}
%	\hfill
%	\subfigure[$\Delta^-(t)$(ABF)]{  
%		\includegraphics[width = 0.66\columnwidth]{dmABF.eps}}
%	\caption{Comparison of time to convergence between GABF and ABF for 100 runs. In (a) and (b), $\delta = M = \sqrt{17}$km and $D = 0$. In (c) and (d), $\delta = M = \sqrt{17}$ km and $D = (\cD(\cG) + \cD(\cG) - 2)e_{\min}$, $e_{\min}$ in those 100 trials are ranging from $9.8 \times 10^{-5}$km to $7.7\times 10^{-3}$km. }
%	\label{fig:comparison}
%\end{figure*} 



%For perturbations, we consider static nodes with asymmetric noise in the estimated $e_{ij}$, then edge lengths in (\ref{dt}) change from their nominal value $e_{ij}$ as $\bar{e}_{ij}(t) = e_{ij} + \epsilon_{ij}(t)$, and $\epsilon_{ij}(t)$ obeys
%\begin{equation}\label{ebound}
%|\epsilon_{ij}(t)| < \epsilon < e_{\min},
%\end{equation} 
%ensuring no edge length is negative. Further, the noise is asymmetric, i.e., $e_{ij}(t) \neq e_{ji}(t)$. In all simulations, $\epsilon_{ij} \in \cU(-\epsilon,\epsilon)$ with $\epsilon = e_{\min}$. $D, M$ and $\delta$ in GABF are set as $D = (\cD(\cG) + \cD(\cG^-) - 2)\epsilon$ and $M = \delta = \sqrt{17}$ km, in which case $\Delta^+(t)$ and $\Delta^-(t)$ in GABF will have the same ultimate bounds as in ABF according to our Theorem \ref{bound}. 
%Figure \ref{fig:comparison} depicts the convergence process of ABF and GABF from the perspective of $\Delta^+(t)$ and $\Delta^-(t)$, the effective diameter for those 100 trials ranges from 15 to 27. Figure \ref{fig:comparison} (a) and (b) show that $\Delta^+(t)$ in ABF converges within $\cD(\cG)$ rounds, while $\Delta^-(t)$, constrained by the "rising value problem" (two nodes with underestimated distance estimates will experience slow convergence resulted from the small edge length between them), takes much longer time to converge, and the average convergence time for those 100 trials is 792 rounds. For GABF, as shown in Figure \ref{fig:comparison} (a) and (b), $\Delta^-(t)$, benefited from the introduced parameters $M$, $\delta$ and $D$, is rid of the "rising value problem" and converges with 2 rounds. Even though the greatest overestimate $\Delta^+(t)$ experiences up and downs and needs a slightly longer time to converge, the total convergence time in GABF is 26 rounds on average, which has significant improvement as compared to GABF.
%For the robustness of GABF and ABF under perturbations. We randomly pick 5 trials and apply the perturbations described above. As shown in Figure \ref{fig:comparison_per}, $\Delta^+(t)$ and $\Delta^-(t)$ in both ABF and GABF will have the same ultimate bounds, which confirms our Theorem \ref{bound}.
\iffalse
\begin{figure}[h]
	\centering
	\subfigure[$\Delta^+(t)$(GABF under perturbations)]{
		\includegraphics[width = 0.85\columnwidth]{dpgabfp.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$(GABF under perturbations)]{  
		\includegraphics[width = 0.85\columnwidth]{dmgabfp.pdf}}
	\vfill
	\subfigure[$\Delta^+(t)$(ABF under perturbations)]{
		\includegraphics[width = 0.85\columnwidth]{dpabfp.pdf}}
	\vfill
	\subfigure[$\Delta^-(t)$(ABF under perturbations)]{  
		\includegraphics[width = 0.85\columnwidth]{dmabfp.pdf}}
	\caption{Comparison of robustness between GABF and ABF for 100 runs of 500 nodes randomly distributed in a $4 \times 1$ $\mathrm{km}^2$ area, showing that both GABF and ABF have the same ultimate bounds.}
	\label{fig:comparison_per}
\end{figure} 
\fi
